DreamTeacher: Pretraining Image Backbones with Deep Generative Models

In this work, we introduce a self-supervised feature representation learning framework DreamTeacher that utilizes generative networks for pre-training downstream image backbones. We propose to distill knowledge from a trained generative model into standard image backbones that have been well engineered for specific perception tasks. We investigate two types of knowledge distillation: 1) distilling learned generative features onto target image backbones as an alternative to pretraining these backbones on large labeled datasets such as ImageNet, and 2) distilling labels obtained from generative networks with task heads onto logits of target backbones. We perform extensive analyses on multiple generative models, dense prediction benchmarks, and several pre-training regimes. We empirically find that our DreamTeacher significantly outperforms existing self-supervised representation learning approaches across the board. Unsupervised ImageNet pre-training with DreamTeacher leads to significant improvements over ImageNet classification pre-training on downstream datasets, showcasing generative models, and diffusion generative models specifically, as a promising approach to representation learning on large, diverse datasets without requiring manual annotation.

==> figs/bdd-feat-viz.tex <==
\begin{figure*}[hbt!]
\vspace{-1mm}
\begin{minipage}{0.48\textwidth}
\begin{center}
\includegraphics[width=0.95\linewidth]{figs/bdd100k-kmean.pdf}
\end{center}
\vspace{-5mm}
\caption{\textbf{\footnotesize K-means clustering of StyleGAN2's features trained on BDD100K.} We run kmeans clustering ($k=10$) on 10k sampled features, and show unsupervised segmentation maps on sampled images. Notice that the clusters are consistent across images (car, sky, tree etc), indicating a semantic meaning of the generative features.
}
\label{fig:stylegan-kmean}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\begin{center}
\includegraphics[width=1\linewidth]{figs/bdd100k-adm-feat-viz.pdf}
\end{center}
\vspace{-5mm}
\caption{\textbf{\footnotesize ADM feature visualization on BDD100k.}
BDD100k image is first diffused by 50 steps and we run one denoising step of the ADM model to extract the feature. We see that features in the low resolution block focus on scene layouts and objects, and in higher resolution, they focus on parts like car wheels, and traffic lights.
}
\label{fig:ddpm-feat}
\end{minipage}
\vspace{-4mm}
\end{figure*}


==> figs/ddpm-bdd100k-feats.tex <==
\begin{figure}[t]
\vspace{-1mm}
\begin{center}
\includegraphics[width=1\linewidth]{figs/bdd100k-adm-feat-viz.pdf}
\end{center}
\vspace{-5mm}
\caption{\textbf{\footnotesize ADM feature visualization on BDD100k.}
BDD100k image is first diffused by 50 steps and we run one denoising step of the ADM model to extract the feature. We see that features in the low resolution block focus on scene layouts and objects, and in higher resolution, they focus on parts like car wheels, and traffic lights.
}
\label{fig:ddpm-bdd-feat}
\vspace{-4mm}
\end{figure}


==> figs/label-efficient-result-viz.tex <==
\newcommand\hhaa{1.5cm}
\newcommand\wwaa{1.5cm}

\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{1pt}
\resizebox{0.96\textwidth }{!}{ %< auto-adjusts
\begin{tabular}{*{13}c}
\rot{\scriptsize{FFHQ-34}} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/IMG_img00000829.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/GT_img00000829.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/img00000829.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/IMG_img00001927.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/GT_img00001927.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/img00001927.png} &
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/IMG_img00015815.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/GT_img00015815.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/img00015815.png} &
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/IMG_img00036478.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/GT_img00036478.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/ffhq/img00036478.png}  \\

\rot{\scriptsize{Bedroom-28 }} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/IMG_bedroom_0000241.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/GT_bedroom_0000241.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/bedroom_0000241.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/IMG_bedroom_0000193.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/GT_bedroom_0000193.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/bedroom_0000193.png} &
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/IMG_bedroom_0000261.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/GT_bedroom_0000261.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/bedroom_0000261.png} &
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/IMG_bedroom_0000249.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/GT_bedroom_0000249.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/bedroom/bedroom_0000249.png}  \\

\rot{\scriptsize{Cat-15}} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/IMG_cat_0000066.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/GT_cat_0000066.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/cat_0000066.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/IMG_cat_0000001.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/GT_cat_0000001.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/cat_0000001.png} &
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/IMG_cat_0000097.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/GT_cat_0000097.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/cat_0000097.png} &
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/IMG_cat_0000062.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/GT_cat_0000062.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/cat/cat_0000062.png}  \\


\rot{\scriptsize{Horse-21}} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/IMG_horse_0000003.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/GT_horse_0000003.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/horse_0000003.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/IMG_horse_0000007.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/GT_horse_0000007.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/horse_0000007.png} &
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/IMG_horse_0000031.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/GT_horse_0000031.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/horse_0000031.png} &
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/IMG_horse_0000040.png} & \includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/GT_horse_0000040.png} & 
\includegraphics[height=\hhaa,width=\wwaa, trim=0 0 0 0,clip]{figs/adm/horse/horse_0000040.png}  \\

&\scriptsize{Image} &  \scriptsize{GT} &  \scriptsize{Dream Teach. } &  \scriptsize{Image} &  \scriptsize{GT} &  \scriptsize{Dream Teach. } & 
\scriptsize{Image} &  \scriptsize{GT} &  \scriptsize{Dream Teach. } &  \scriptsize{Image} &  \scriptsize{GT} &  \scriptsize{Dream Teach. } \\



% \rot{\scriptsize{Semantic Seg.}}&\includegraphics[height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/bdd/img-seg_1.jpg} &
% \includegraphics[height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/bdd/densecl-IN-seg_1.jpg} & 
% \includegraphics[height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/bdd/dt-bdd100k-seg_1.jpg} &
% \includegraphics[height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/bdd/dt-IN-seg_1.jpg} \\
% &\scriptsize{Image} &  \scriptsize{denseCL IN-1k-1M pre-trained} &  \scriptsize{DT-feat.distil. BDD100K pre-trained } &  \scriptsize{DT-feat.distil. IN-1k-1M pre-trained }  \\

\end{tabular}}
\vspace{-3mm}
\caption{\textbf{Qualitative results on Label-efficient benchmarks.}  We visualize predictions from {\ourmodel} with ADM generator using mix-distillation to a ConvNX-B backbone. Our predictions are accurate, even on thin structures like cat's whiskers. % and bedroom furniture with a comparison to the ground truth(GT). %It also works well will multi object scenes in horse class. 
}
\label{tab:top5-analysis}
\vspace{-4mm}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/bdd_per_class.tex <==
%\newcommand*\rot{\rotatebox{90}}
\begin{table*}[t]
\centering
\resizebox{0.9\textwidth }{!}{ %< auto-adjusts font size to fill line
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} ll*{20}l @{}}
 Method & pre-data
 & \rot{~Road} 
 & \rot{Sidew.}
 & \rot{Bldg.}
 & \rot{Wall}
 & \rot{Fence}
 & \rot{Pole}
 & \rot{Light}
 & \rot{Sign}
 & \rot{Veget.}
 & \rot{Terrain}
 & \rot{Sky}
 & \rot{Person}
 & \rot{Rider}
 & \rot{Car} 
 & \rot{Truck}
 & \rot{Bus}
 & \rot{Train}
 & \rot{Mcycle}
 & \rot{Bicycle}
 & \rot{mIoU} \\
\hline
IN sup. & IN1k-1M & 95.0 & 67.3 & 87.1 & 30.7 & \textbf{54.9} & 56.7& 61.1& 60.5& 87.5& 50.3& 95.7& 66.3& 24.9& 90.9& 56.2& 82.0& 0.0& \textbf{57.1} & \textbf{55.6} & 62.1\\
\hline
denseCL & IN1k-1M & 95.3 & \textbf{68.7} & 87.1 & 32.5 & 49.6 & 55.7 & \textbf{61.9}& \textbf{61.2}& 87.1& 47.4 & 95.7& 65.5& 25.1& 91.1& 56.1& \textbf{83.9}& 0.0& 43.2 & 48.4 & 60.8\\

DT-feat.distil. & IN1k-1M & 95.3 & 67.6 & \textbf{87.7} & \textbf{35.6} & 53.2 & \textbf{57.3}& 61.4& 60.8& \textbf{87.7}& \textbf{51.5}& 95.7& \textbf{68.4}& \textbf{33.5}& 91.4& 59.4& 82.0& 0.0& 48.0 & 51.8 & \textbf{62.6}\\

DT-feat.distil. & BDD100K & \textbf{95.3} & 68.5 & 87.0 & 33.1 & 54.0 & 56.2& 61.1 & 59.1& 87.2& 48.6& \textbf{95.7}& 65.5& 16.6& \textbf{91.4}& \textbf{59.6}& 82.1& 0.0& 40.3 & 45.3 & 60.3\\

\hline

\end{tabular}}
\vspace{-3mm}
\caption{
% 
\textbf{BDD100k sem. seg. per-class performance.} %We compare strong self-supervised denseCL pre-trained on ImageNet as well as supervised pre-trained backbone with class labels. 
Backbone is ResNet50 for all methods. We highlight several important observations: 1) when pre-trained on ImageNet without labels (third row), our method outperforms an ImageNet pre-trained variant (first row) -- an important result for the representation learning domain. 2) When pre-training on a complex target domain (AV dataset), unsupervised pre-training is still behind ImageNet pre-training. There are clear performance drops for motorbike, rider and bicycle, which are all less frequent objects. This warrants further investigation on larger datasets. 3) We outperform a SOTA baseline (second row) when pre-training on ImageNet. 
%Our DT-feat.distil. achieves the best overall mIoU 62.6 without using any labels for pre-training, outperforming denseCL by 1.8 percent. We also include our DT-feat.distil. pre-trained on BDD100K unlabeled images. We find that in-domain pre-training achieves competitive performance on thing class like road and side walk and common objects like car (91.4) and truck(59.6), but not good at rare objects like rider. Interestingly, supervised pre-trained method with ImageNet class labels perform much better in rare classes Motocylce and bicycle, comparing to unsupervised methods. 
% 
} % \caption
\label{tab:perclassbdd}
\vspace{-4mm}
\end{table*}

==> tables/bdd_pose.tex <==
\begin{table*}[h]
\vspace{-2mm}
\centering
\resizebox{0.8\textwidth }{!}{ %< auto-adjusts font size to fill line
\setlength{\tabcolsep}{14pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|c|c}
pre-train & backbone  & pre-data &  AP \\
\hline
Random init.  & HRNet-w48 & - & 48.56\\

Classification & HRNet-w48 & IN1k-1M & 50.16 \\
\hline

Ours   & HRNet-w48&  Nuscene-crop + BDD100k-crop & 50.54 \\
Classification + Ours   & HRNet-w48 & IN1k-1M  + Nuscene-crop + BDD100k-crop & \textbf{51.17} \\



\end{tabular}}


\caption{
% 
\textbf{Pose Estimation on BDD100K} 
% 
} % \caption
\label{tab:cityscape-voc}
\vspace{-4mm}
\end{table*}

==> tables/bdd_pretrain.tex <==
\begin{table*}[htb!]
\vspace{-0.5mm}

\centering
\resizebox{0.94\textwidth }{!}{ %< auto-adjusts font size to fill line
\setlength{\tabcolsep}{9pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lccccccccc}
\toprule
& & & &\multicolumn{1}{c}{\textbf{Semantic Seg.}} & \multicolumn{2}{c}{\textbf{Instance Seg.}} & \multicolumn{3}{c}{\textbf{Panoptic Seg.}}\\
pre-train & backbone & pre-data & pre-epoch & \textit{mIoU} &\textit{Box mAP} & \textit{Mask mAP} & $PQ$ & $PQ^{th}$ & $PQ^{st}$\\
\midrule
random init. & RN50 & - & -&53.8 & 17.5 & 15.6 & 12.2 & 9.5 & 13.1\\
sup.   & RN50 & IN1k-1M & -&62.1 & 26.1 & 20.2 & 22.4 & 27.9 & 20.5\\
\midrule
% MAE\cite{he2022masked} & ViT-b & BDD100K & 400 & 56.3 & -& -& -&-&-\\
% MAE\cite{he2022masked} & ViT-b & BDD100K & 1600 & 58.9 & -& -& -&-&-\\
% \midrule
%SimCLR & RN50 & IN1k & ? & 38.7& 34.9& ?& ?\\
BYOL\cite{grill2020bootstrap} & RN50 & BDD100K & 200 & 55.3 & 20.4& 17.8& 19.3&23.6&17.8\\
SwAV\cite{caron2020unsupervised} & RN50 & BDD100K & 200 & 56.0 & 19.8& 17.1& 19.0&23.9&17.4\\
denseCL\cite{wang2021dense} & RN50 & BDD100K & 200 & 57.9 & 21.5& 18.9& 20.4&25.5&18.6\\
MoCoV2\cite{chen2020improved} & RN50 & BDD100K & 200 & 58.5 & 22.2& 19.3& 20.1&24.6&18.6\\
DT-feat.distil. w/ StyleGAN2\cite{karras2020analyzing} & RN50 & BDD100K & 200 & \textbf{60.3} & 25.1& 21.4& 21.5& \textbf{27.4} &19.5\\
DT-feat.distil. w/ ADM\cite{dhariwal2021diffusion} & RN50 & BDD100K & 200 & 59.5& 25.0& 21.9& 21.5 & 26.7 & 19.8\\
\midrule
DT-feat.distil. w/ ADM\cite{dhariwal2021diffusion} & RN50 & BDD100K & 600 & \textbf{60.3}& \textbf{26.3}& \textbf{23.4}& \textbf{21.8}& 27.1& \textbf{20.0}\\

\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{
% 
\textbf{BDD100K in-domain pre-training benchmark.} We compare SoTA self-supervised baselines including recently proposed MAE with the ViT-b architecture. We pretrain all methods on the BDD100K dataset without labels, and finetune the backbone on semantic/instance/panoptic segmentation tasks. Our methods %with the same pre-training epoch 
beat all baselines on all three tasks. %Our DT-feat.distil. with  StyleGAN2 generator achieves the best performance in semantic segmentation and the best $PQ^{th}$ in panoptic segmentation. Our DT-feat.distil. with the diffusion generative model achieves 26.3 \textit{Box mAP} and 23.4 \textit{Mask mAP} higher than the best performing baseline MoCoV2 by 4 points.
% 
} % \caption
\label{bdd100k_indomain}
\vspace{-4mm}
\end{table*}

==> tables/bdd_readout.tex <==
\begin{table}[h]
\centering
\resizebox{0.3\textwidth }{!}{ %< auto-adjusts font size to fill line
\setlength{\tabcolsep}{14pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{l|c|c}
Method & backbone &\textit{mIoU} \\
\hline
SwAV & RN50 & 31.9  \\
denseCL & RN50 & 32.2  \\
MocoV2 & RN50 & 34.5 \\
BYOL & RN50 & 35.5 \\
%MAE & ViT-b & ? \\
\hline
Ours & RN50 & \textbf{38.8} \\
\end{tabular}}

\caption{
% 
\textbf{BDD100k Semantic Segmentation with backbone freeze and only finetune the head (readout)} 
% 
} % \caption

\end{table}

==> tables/bdd_scale_data.tex <==
\begin{table}[h]
\centering
\resizebox{0.9\linewidth }{!}{ %< auto-adjusts font size to fill line
\setlength{\tabcolsep}{12pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{l|c|ccc}
Method & backbone &$PQ$ & $PQ^{th}$ & $PQ^{st}$ \\
\hline
sup & IN1M & 22.4&27.9&20.5  \\
\hline
ours & BDD100K & 21.8&27.1&20.0  \\
ours & BDD3M & 22.1& 28.2&20.0\\
\end{tabular}}
\vspace{-2mm}
\caption{
% 
\textbf{Scale up dataset size.} We scale unlabeled image size from 100k to 3M and show downstream performance on BDD100K panoptic segmentation. 
% 
} % \caption
\vspace{-1mm}
\end{table}

==> tables/cityscape_ssl.tex <==
\begin{table*}[h]
\centering
\resizebox{0.7\textwidth }{!}{ %< auto-adjusts font size to fill line
\setlength{\tabcolsep}{16pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lccccc}
method & backbone & 1(2,975) & 1/4(744) & 1/8(372) & 1/30(100)\\
\hline
%classific. sup. & RN50 & 78.7 & 71.3 & 65.4 & 54.4 \\
classific. sup. & RN101 & 79.7 & 71.8 & 66.2 & 57.8 \\
% \hline
% \multicolumn{3}{l}{\textit{Methods using general-domain unlabeled data(imagenet) in a task-agnostic way:}} \\
% BYOL & RN50 & IN1k-1M & 77.9 & 68.6 & 63.8 & 55.6 \\ 
% MocoV2 & RN50 & IN1k-1M & 77.1 & 70.6 & 66.4 & 54.2 \\ 
% DDPM feat.distil (ours) & RN50 & IN1k-1M & \textbf{78.8} & ? & ? & ? \\ 
% \hline
% \multicolumn{3}{l}{\textit{Methods using in-domain(driving) unlabeled data in a task-agnostic way:}} \\
% BYOL & RN50 & BDD100k & 72.4 & 50.8 & 49.8 & 42.6 \\ 
% MocoV2 & RN50 & BDD100k & 74.9 & 61.3 & 56.4 & 46.3 \\ 
% DDPM feat.distil (ours) & RN50 & BDD100k & \textbf{75.0} & \textbf{63.1} & \textbf{60.0} & \textbf{50.0} \\ 
\hline
%\multicolumn{3}{l}{\textit{Methods using in-domain(driving) unlabeled data in a task-specific way:}} \\
AdvSemSeg & RN101  & - & 62.3 & 58.8 & - \\  
s4GAN & RN101  & 65.8 & 61.9 & 59.3 & - \\  
DMT & RN101  & 68.2 & - & 63.0 & 54.8 \\  
ClassMix & RN101  & - & 63.6 & 61.4 & - \\  
CutMix & RN101  & - & 68.3 & 65.8 & 55.7 \\  
PseudoSeg & RN101 & - & 72.4 & 69.8 & 61.0 \\  
%PC2Seg & RN50  & 75.4 & 73.8 & 72.1 & 60.4 \\  
PC2Seg & RN101  & 76.0 & 75.2 & 72.3 & 62.9 \\  
\hline
stylegan2-feat.distil. (ours) & RN101 & \textbf{80.2} & 74.0 & 69.2 & 60.1 \\ 
adm-mix.distil. (ours) & RN101 & ? & ? & ? & ? \\ 
\end{tabular}}

\caption{
% 
\textbf{Cityscapes semantic segmentation benchmark in a semi-supervised setup.} 
% 
} % \caption

\end{table*}




==> tables/in_transfer.tex <==
\begin{table}[htb!]
\vspace{-0mm}
\centering
\resizebox{1.0\linewidth }{!}{ %< auto-adjusts font size to fill line
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lccccc}
\toprule
&  \multicolumn{1}{c}{\textbf{ADE20k Seg.}} & \multicolumn{2}{c}{\textbf{MS-COCO Ins. Seg}} & \multicolumn{2}{c}{\textbf{BDD100k Ins. Seg}}\\
pre-train & \textit{mIoU} &\textit{Box mAP} & \textit{Mask mAP} & \textit{Box mAP} & \textit{Mask mAP}\\
\midrule
% MAE & ViT-B & IN1k &  ? &  ? &  ? & ? & ? \\
% \hline \hline
random init. & 32.8 & 31.0 & 28.3 & 17.5 & 15.6 \\
supervised.  & 40.9 & 40.4 & 36.3 & 26.1 & 20.2\\
SimCLR\cite{chen2020simple} & 39.9 & 38.7& 34.9& 24.5& 20.6\\
denseCL\cite{wang2021dense} & 41.1 & 40.3& 36.4& 27.1& 23.4 \\
MocoV2\cite{chen2020improved} & 40.9 & 40.2& 36.1& 26.9& 22.9\\
SimSiam\cite{chen2021exploring} & 40.6 & 38.8& 34.9& 26.3& 22.7\\
SwAV\cite{caron2020unsupervised}& 41.2 & 40.2& 36.3& 25.6&22.2\\
BYOL\cite{grill2020bootstrap} & 41.6 & 40.9& 36.8& 26.2&22.6\\
PixPro\cite{} & 41.6 & 40.7& 36.6& 27.2&23.1\\
SparK\cite{} & ? & ? & ? & 25.7 & 22.4\\
\midrule
DT-feat.distil. w/ BigGAN\cite{brock2018large}  & 40.8& 38.4& 34.5& 24.9&21.2\\
DT-feat.distil. w/ ICGAN\cite{casanova2021instance}  & 41.2 & 38.3& 34.6& 26.3&22.2\\
DT-feat.distil. w/ ADM\cite{dhariwal2021diffusion} & \textbf{42.5}& \textbf{41.2}& \textbf{37.4}& \textbf{28.3} & \textbf{24.8}\\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{
% 
\textbf{\footnotesize Transfer learning using ImageNet.} All methods pretrain ResNet50 for 200 epochs on ImageNet-1M, without labels. Only the backbone is then finetuned on downstream datasets. Here we use feature distillation with online sampling with two unconditional GANs, and encode real images with diffusion generative model ADM without classifier-guidance. Our DT with ADM beats baselines including the supervised ImageNet pre-trained backbone, showing strong transfer performance for dense prediction tasks.
% 
} % \caption

\vspace{-4mm}
\label{IN_transfer}
\end{table}





==> tables/in_transfer_ade-bdd.tex <==
\begin{table}[htb!]
\vspace{-0mm}
\centering
\resizebox{1.0\linewidth }{!}{ %< auto-adjusts font size to fill line
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{l|ccc}
\toprule
\multirow{2}{*}{Pre-training (ResNet-50)}&  \multicolumn{1}{c}{ADE20k} & \multicolumn{2}{c}{BDD100k}\\
& mIoU & AP$^{bb}$ & AP$^{mk}$\\
\midrule
% MAE & ViT-B & IN1k &  ? &  ? &  ? & ? & ? \\
% \hline \hline
%random init. & 32.8 & 31.0 & 28.3 & 17.5 & 15.6 \\
Supervised \cite{yu2020bdd100k}  & 40.9 & 26.1 & 20.2\\
SimCLR\cite{chen2020simple} & 39.9 & 24.5& 20.6\\
SparK\cite{tov2021designing} & 40.5 & 25.7 & 22.4\\
SimSiam\cite{chen2021exploring} & 40.6 & 26.3& 22.7\\
MoCov2\cite{chen2020improved} & 40.9 & 26.9& 22.9\\
denseCL\cite{wang2021dense} & 41.1 & 27.1& 23.4 \\
SwAV\cite{caron2020unsupervised}& 41.2 & 25.6&22.2\\
BYOL\cite{grill2020bootstrap} & 41.6 & 26.2&22.6\\
PixPro\cite{xie2021propagate} & 41.6 & 27.2&23.1\\

%\midrule
% DT-feat.distil. w/ BigGAN\cite{brock2018large}  & 40.8& 38.4& 34.5& 24.9&21.2\\
% DT-feat.distil. w/ ICGAN\cite{casanova2021instance}  & 41.2 & 38.3& 34.6& 26.3&22.2\\
\rowcolor{LightBlue}
DT-feat.distil. w/ ADM\cite{dhariwal2021diffusion} & \textbf{42.5}& \textbf{28.3} & \textbf{24.8}\\

\bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{
% 
\textbf{\footnotesize Transfer learning: ADE20k and BDD100k.} All methods are pre-trained on IN-1k and fine-tuned on downstream tasks. For ADE20k, we follow \cite{} to use UperNet as segmentation method, reported number is mean IoU at single scale. For BDD100k, we follow \cite{yu2020bdd100k} official setup to use Mask R-CNN ResNet50-FPN fine-tuned for 36 (3x) epochs.
% 
} % \caption

\vspace{-4mm}
\label{IN_transfer}
\end{table}

==> tables/label_efficient_benchmark.tex <==
\begin{table*}[htb!]
\vspace{-0.5mm}
\centering
\resizebox{0.94\textwidth }{!}{ %< auto-adjusts font size to fill line
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lccccccc}
\toprule
method & backbone & params & pre-data & Bedroom-28 & FFHQ-34 & Cat-15 & Horse-21\\
\midrule
classific. sup. & RN101 & 43M & IN1k-1M & 34.4 & 53.6 & 38.8 & 51.1 \\
classific. sup. & ConvNX-B & 89M & IN21k-14M & 41.0 & 59.2 & 47.3 & 56.0 \\
%classific. sup. & Swin-L & 197M & IN21k-14M & 42.3 & 57.3 & 47.6 & 57.7 \\
% \midrule
% ALAE\cite{pidhorskyi2020adversarial} & Custom & - & task domains & 20.0 & 48.1 & - & - \\  
% VDVAE\cite{child2020very} & Custom & 115M & task domains & - & 57.3 & - & - \\
% GAN Inv.\cite{tov2021designing} & Custom & -& task domains & 13.9 & 51.7 & 21.4 & 17.7  \\
% GAN Enc. & Custom & -& task domains & 22.4 & 53.9 & 32.0 & 26.7  \\
\midrule
SwAV\cite{caron2020unsupervised} & RN50-w2 & 94M& task domains & 41.0 & 54.7 & 44.1 & 51.7  \\
MAE\cite{he2022masked} & ViT-L & 305M & task domains & 45.0 & 58.8 & 52.4 & 63.4  \\
DatasetGAN\cite{zhang2021datasetgan} & RN101 & 43M & task domains & 31.3 & 57.0 & 36.5 & 45.4  \\
DatasetDDPM\cite{baranchuk2021labelefficient}  & RN101 & 43M & task domains & 47.9 & 56.0 & 47.6 & 60.8 \\
DDPM-seg\cite{baranchuk2021labelefficient}   & UNet & 554M & task domains & 49.4  & 59.1 & 53.7 & 65.0 \\
% DDPM-seg(our interp.) \\ \HUAN{do we need to discuss this in main text?}& UNet & 554M & task domains &  49.8 & 60.1 & 57.6 & 64.0 \\
%DDPM-seg(our interp.)& UNet & 554M & IN1k-1M & 34.3 & 59.2 & 49.8 & 56.6 \\
%DT-mix.distil.deter.(ours)& RN101 & 43M & task domains& 44.7  & 57.8 & 50.9 & 59.9 \\


%DT-feat.distil.(ours)& ConvNX-B & 89M & task domains& 53.1 & 61.1 & 58.2 & 64.7 \\
%DT-label.distil.(ours)& ConvNX-B & 89M & task domains& \textbf{54.6}  & \textbf{61.5} & \textbf{58.6} & 64.4 \\
\rowcolor{LightBlue}
DT-mix.distil. w/ ADM\cite{dhariwal2021diffusion}& RN101 & 43M & task domains&  49.9  &  59.4 & 56.7 &  65.9 \\
\rowcolor{LightBlue}
DT-mix.distil. w/ ADM\cite{dhariwal2021diffusion}& ConvNX-B & 89M & task domains& \textbf{54.8}  & \textbf{61.2} & \textbf{58.6} & \textbf{67.6} \\
\bottomrule
%DT-label.distil.(ours)& Swin-L & 197M & task domains& ?  & ?& ? & ? \\
\end{tabular}}
\vspace{-2.5mm}
\caption{
% 
\textbf{Label-efficient semantic segmentation benchmark.} We compare our {\ourmodel} (DT) with various representation learning baselines. %including VAE based ALAE, VDVAE, and GAN inversion with auxiliary encoder, GAN Inv. GAN Enc. as well as unsupervised representation learning SwAV and MAE and semi-supervised baselines DatasetGAN, DatasetDDPM. Also previous SoTA DDPM-seg. 
Our \emph{DT-mix.distil.} with ResNet 101 backbone (only 43M parameters) beats all baselines, some with 10x the number of parameters. We also show our method with ConvNX-B achieves the new SoTA without using any extra data, i.e. IN1k-1M or IN21k-14M.  
% 
} % \caption
\label{label-efficient}
\vspace{-2mm}
\end{table*}

% \begin{table*}[h]
% \centering
% \resizebox{0.7\textwidth }{!}{ %< auto-adjusts font size to fill line
% \setlength{\tabcolsep}{14pt}
% \renewcommand{\arraystretch}{1.0}
% \begin{tabular}{l|c|c|c|c}
% encoding  & Bedroom-28 & FFHQ-34 & Cat-15 & Horse-21\\
% \hline
% Deterministic & 44.7  & 57.8 & 50.9 & 59.9 \\
% Stochastic & ? & ? & ? & ? \\
% \end{tabular}}

% \caption{
% % 
% \textbf{Ablation study on different DDPM encoding scheme.} We use the same backbone ResNet101 and pretraining using our mix distillation method. Since deterministic encoding training is slow, here we choose to pretrain both method with 30 epochs.
% % 
% } % \caption
% \end{table*}


